Chiral Effective Field Theory and the High-Density Nuclear Equation of State

Born in the aftermath of core collapse supernovae, neutron stars contain matter under extraordinary conditions of density and temperature that are difficult to reproduce in the laboratory. In recent years, neutron star observations have begun to yield novel insights into the nature of strongly interacting matter in the high-density regime where current theoretical models are challenged. At the same time, chiral effective field theory has developed into a powerful framework to study nuclear matter properties with quantified uncertainties in the moderate-density regime for modeling neutron stars. In this article, we review recent developments in chiral effective field theory and focus on many-body perturbation theory as a computationally efficient tool for calculating the properties of hot and dense nuclear matter. We also demonstrate how effective field theory enables statistically meaningful comparisons between nuclear theory predictions, nuclear experiments, and observational constraints on the nuclear equation of state.

==> diagrams/2nd_order_anomalous <==
\begin{fmffile}{diag_2nd_order_anomalous}
	\begin{fmfgraph*}(30,50)
		\fmfcmd{style_def half_prop expr p =
			draw_plain p;
			shrink(.7);
			cfill (marrow (p, .5))
			endshrink;
			enddef;
		}
		\fmftop{v1}\fmfbottom{v0}
		\fmfv{d.shape=circle,d.filled=full,d.size=2thick}{v0}
		\fmfv{d.shape=circle,d.filled=full,d.size=2thick}{v1}
		\fmffreeze
		\fmf{fermion,tension=1.35}{v1,v1}
		\fmf{fermion,tension=1.35}{v0,v0}
		\fmf{half_prop,right=0.5}{v1,v0}
		\fmf{half_prop,right=0.5}{v0,v1}
	\end{fmfgraph*}
\end{fmffile}


==> diagrams/3rd_order_hh <==
\begin{fmffile}{diag_3rd_order_hh}
	\begin{fmfgraph*}(30,40)
		\fmfcmd{style_def half_prop expr p =
			draw_plain p;
			shrink(.7);
			cfill (marrow (p, .5))
			endshrink;
			enddef;
		}
		\fmftop{v2}\fmfbottom{v0}
		\fmfv{d.shape=circle,d.filled=full,d.size=2thick}{v0}
		\fmfv{d.shape=circle,d.filled=full,d.size=2thick}{v1}
		\fmfv{d.shape=circle,d.filled=full,d.size=2thick}{v2}
		\fmffreeze
		\fmf{half_prop,right=0.5}{v1,v0}
		\fmf{half_prop,left=0.5}{v1,v0}
		\fmf{half_prop,right=0.5}{v2,v1}
		\fmf{half_prop,left=0.5}{v2,v1}
		\fmf{half_prop,right=0.5}{v0,v2}
		\fmf{half_prop,left=0.5}{v0,v2}
	\end{fmfgraph*}
\end{fmffile}


==> diagrams/3rd_order_ph <==
\begin{fmffile}{diag_3rd_order_ph}
	\begin{fmfgraph*}(30,40)
		\fmfcmd{style_def half_prop expr p =
			draw_plain p;
			shrink(.7);
			cfill (marrow (p, .5))
			endshrink;
			enddef;
		}
		\fmftop{v2}\fmfbottom{v0}
		\fmfv{d.shape=circle,d.filled=full,d.size=2thick}{v0}
		\fmfv{d.shape=circle,d.filled=full,d.size=2thick}{v1}
		\fmfv{d.shape=circle,d.filled=full,d.size=2thick}{v2}
		\fmffreeze
		\fmf{half_prop,right=0.5}{v1,v0}
		\fmf{half_prop,right=0.5}{v0,v1}
		\fmf{half_prop,right=0.5}{v2,v1}
		\fmf{half_prop,right=0.5}{v1,v2}
		\fmf{half_prop,right=0.5}{v2,v0}
		\fmf{half_prop,right=0.5}{v0,v2}
	\end{fmfgraph*}
\end{fmffile}

